Learning Bipedal Robot Locomotion from Human Movement

Teaching an anthropomorphic robot from human example offers the opportunity to impart humanlike qualities on its movement. In this work we present a reinforcement learning based method for teaching a real world bipedal robot to perform movements directly from human motion capture data. Our method seamlessly transitions from training in a simulation environment to executing on a physical robot without requiring any real world training iterations or offline steps. To overcome the disparity in joint configurations between the robot and the motion capture actor, our method incorporates motion re-targeting into the training process. Domain randomization techniques are used to compensate for the differences between the simulated and physical systems. We demonstrate our method on an internally developed humanoid robot with movements ranging from a dynamic walk cycle to complex balancing and waving. Our controller preserves the style imparted by the motion capture data and exhibits graceful failure modes resulting in safe operation for the robot. This work was performed for research purposes only.

==> model_description.tex <==

In this work we consider a robot as a human-like mechanism controlled via actuators.  Our goal is to train a neural network to generate a series of commands for the actuators which guide the robot through a target motion.  We utilize a dynamics simulation environment to model the mechanical response of the actuators to the control input.  The dynamical properties of the rigid bodies are fully described by their individual mass and inertia tensors.  The geometric shape of each body part is modeled by fitting a collision volume to the underlying mesh.  Body parts are considered to be interacting when the associated collision volumes intersect in space.  This interaction is simulated in a physically realistic way by applying normal reaction and dry friction forces.  The reaction force is defined by the mutual penetration depth of the collision volumes.  The dry friction force is defined as 
$\vec{F} = -k \frac{\vec{v}}{\vert \vec{v} \vert } \vert \vec{F_{react}} \vert$, where $\vec{F}$ is friction force,  $k$ - friction coefficient, $\vec{v}$ is relative velocity,and $\vec{F_{react}}$ surface interaction reaction force.

 

  The robot's body parts are represented as rigid bodies connected via hinge joints.  Each physical joint is equipped with a servo controller which applies torque to the joint when required.  We use the Proportional Integral Differential (PID) regulator model of a servo controller to represent the controllers in simulation.

 

  The robot is equipped with several sensors which it uses to perceive its state in relation to the environment.  These are modeled as virtual sensors in simulation.  The list of sensors is as follows: an Inertia Measurement Unit (IMU) to measure acceleration and angular velocity, joint angle sensors which provide feedback signals to the associated joint servo controllers, foot pressure sensors to measure surface reaction forces, and an internal clock to measure time.  In simulation each sensor reading is the superposition of the idealized reading combined with simulated bias and noise.







